Customizable Contraction Hierarchies -- A Survey

This work establishes the technical fundamentals of a well-tuned Customizable Contraction Hierarchies (CCH) implementation that is simple and elegant. We give a detailed overview of the state of the art of CCH, review recent advances on CCH and show how to combine them. Additionally, we propose further refinements that improve the performance of CCH. An extensive evaluation confirms that a CCH framework is not only comprehensive in supported features but also competitive in performance to both Contraction Hierarchies (CH) and Customizable Route Planning (CRP).

==> table/alt_stats.tex <==
\begin{tabular}{lrrrrr}
\toprule
 & \# Alt. & Success   & Running   & \# Iterations & Sharing \\
 &         & rate [\%] & time [ms] &               &    [\%] \\
\midrule
Stuttgart & 1 &     82.9 &              1.0 &        2.2 &             41.0 \\
       & 2 &     63.9 &              2.4 &        4.1 &             45.9 \\
       & 3 &     48.0 &              4.0 &        5.8 &             51.2 \\
       & 4 &     34.6 &              6.0 &        7.4 &             54.5 \\
\addlinespace Germany & 1 &     95.7 &             97.4 &        1.5 &             34.4 \\
       & 2 &     87.1 &            294.0 &        3.0 &             43.3 \\
       & 3 &     71.3 &            595.2 &        4.3 &             49.2 \\
       & 4 &     53.6 &            973.5 &        5.4 &             52.9 \\
\addlinespace Europe & 1 &     97.3 &            213.4 &        1.4 &             41.9 \\
       & 2 &     91.1 &            548.8 &        2.7 &             47.8 \\
       & 3 &     77.8 &            996.8 &        4.0 &             52.1 \\
       & 4 &     58.7 &           1\,473.9 &        5.1 &             55.1 \\
\bottomrule
\end{tabular}



==> table/bidir.tex <==
\begin{tabular}{ccrrrrrrrr}
\toprule
 &  & \multicolumn{5}{c}{Running time [ms]} & \multicolumn{3}{c}{Queue pushes [$\cdot 10^3$]} \\ \cmidrule(l{3pt}r{3pt}){3-7} \cmidrule(l{3pt}r{3pt}){8-10}\multirow{2}{*}{\lquery} & & \multirow{2}{*}{Zero} & \multirow{2}{*}{ALT} & \multirow{2}{*}{CH} & \multirow{2}{*}{CCH} & \multirow{2}{*}{Oracle} & \multirow{2}{*}{Zero} & \multirow{2}{*}{ALT} & (C)CH/ \\
 & & & & & & & & & Oracle \\
\midrule
\multirow{3}{*}{$\lpre$} & Unidirectional &            584.87 & 43.02 &  0.47 &  0.64 &   0.16 &                    1\,674.35 &  96.21 &         0.66 \\
        & Average &            373.18 & 12.83 &  0.79 &  1.13 &   0.18 &                     916.15 &  23.08 &         0.60 \\
        & Symmetric &            376.72 & 40.19 &  0.69 &  0.92 &   0.19 &                     908.55 &  76.61 &         0.57 \\
\addlinespace
\multirow{3}{*}{$\lpre \cdot 1.05$} & Unidirectional &            580.66 & 90.79 & 15.91 & 18.09 &  10.06 &                    1\,681.39 & 179.66 &        26.78 \\
        & Average &            365.82 & 33.22 & 19.34 & 18.66 &   9.96 &                     916.15 &  57.27 &        23.60 \\
        & Symmetric &            368.94 & 72.67 & 21.54 & 20.39 &  11.22 &                     908.55 & 123.77 &        20.72 \\
\addlinespace
\multirow{3}{*}{\shortstack{$\lpre \cdot 1.5$ if\\ speed \\ < 80kph}} & Unidirectional &            637.24 & 96.62 & 21.78 & 21.37 &  14.62 &                    1\,674.26 & 171.02 &        36.54 \\
        & Average &            361.83 & 19.50 & 10.92 & 10.94 &   5.34 &                     845.06 &  34.03 &        13.25 \\
        & Symmetric &            364.55 & 37.33 & 11.89 & 11.75 &   6.00 &                     836.44 &  57.93 &        11.53 \\
\bottomrule
\end{tabular}



==> table/bidir_pruning.tex <==
\begin{tabular}{c@{\hskip6pt}c@{\hskip3pt}crrrrrrrr}
\toprule
 &  &  & \multicolumn{5}{c}{Running time [ms]} & \multicolumn{3}{c}{Queue pushes [$\cdot 10^3$]} \\ \cmidrule(l{3pt}r{3pt}){4-8} \cmidrule(l{3pt}r{3pt}){9-11}
Low Deg.      & Bidir. & New & \multirow{2}{*}{Zero} & \multirow{2}{*}{ALT} & \multirow{2}{*}{CH} & \multirow{2}{*}{CCH} & \multirow{2}{*}{Oracle} & \multirow{2}{*}{Zero} & \multirow{2}{*}{ALT} & (C)CH/ \\
Opt. & Pot.     & Pruning  & & & & & & & & Oracle \\
\midrule
\xmark & Avg. &            \xmark &           1\,441.41 & 126.46 &  62.61 &  53.91 &  37.29 &                    4\,493.97 &  292.01 &       125.16 \\
\xmark & Avg. &             \cmark &           1\,451.96 & 128.20 &  62.48 &  54.28 &  38.89 &                    4\,491.56 &  290.92 &       125.08 \\
\xmark & Sym. &            \xmark &           5\,779.64 & 795.56 & 122.70 & 111.78 &  88.66 &                   16\,042.82 & 1\,688.60 &       259.78 \\
\xmark & Sym. &             \cmark &           1\,453.58 & 261.80 &  59.22 &  51.97 &  37.37 &                    4\,491.56 &  624.25 &       116.71 \\
\addlinespace
\cmark & Avg. &            \xmark &            365.82 &  33.22 &  19.34 &  18.66 &   9.96 &                     916.15 &   57.27 &        23.60 \\
\cmark & Avg. &             \cmark &            369.51 &  33.37 &  19.54 &  18.88 &   9.98 &                     908.55 &   56.09 &        23.25 \\
\cmark & Sym. &            \xmark &           1\,512.48 & 241.27 &  40.98 &  38.99 &  26.36 &                    3\,317.81 &  334.90 &        44.67 \\
\cmark & Sym. &             \cmark &            368.94 &  72.67 &  21.54 &  20.39 &  11.22 &                     908.55 &  123.77 &        20.72 \\
\bottomrule
\end{tabular}



==> table/bidir_switching.tex <==
\begin{tabular}{cccrrrrrrrr}
\toprule
 &  &  & \multicolumn{5}{c}{Running time [ms]} & \multicolumn{3}{c}{Queue pushes [$\cdot 10^3$]} \\ \cmidrule(l{3pt}r{3pt}){4-8} \cmidrule(l{3pt}r{3pt}){9-11}\multirow{2}{*}{\lquery} & Bidir. & Choose    & \multirow{2}{*}{Zero} & \multirow{2}{*}{ALT} & \multirow{2}{*}{CH} & \multirow{2}{*}{CCH} & \multirow{2}{*}{Oracle} & \multirow{2}{*}{Zero} & \multirow{2}{*}{ALT} & (C)CH/ \\
 & Pot.     & Direction & & & & & & & & Oracle \\
\midrule
\multirow{4}{*}{$\lpre$} &   Avg. &               Alternating &            373.18 & 12.83 &  0.79 &  1.13 &   0.18 &                     916.15 &  23.08 &         0.60 \\
           &   Avg. &                  Min. Key &            406.35 & 13.68 &  1.44 &  1.75 &   0.56 &                     986.40 &  26.39 &         1.15 \\
           & Sym. &               Alternating &            376.72 & 40.19 &  0.69 &  0.92 &   0.19 &                     908.55 &  76.61 &         0.57 \\
           & Sym. &                  Min. Key &            427.51 & 50.46 &  1.77 &  1.99 &   0.83 &                     978.62 &  99.62 &         1.44 \\
\addlinespace
     \multirow{4}{*}{$\lpre \cdot 1.05$} &   Avg. &               Alternating &            365.82 & 33.22 & 19.34 & 18.66 &   9.96 &                     916.15 &  57.27 &        23.60 \\
           &   Avg. &                  Min. Key &            391.70 & 38.06 & 21.76 & 20.44 &  11.30 &                     986.41 &  67.65 &        26.42 \\
           & Sym. &               Alternating &            368.94 & 72.67 & 21.54 & 20.39 &  11.22 &                     908.55 & 123.77 &        20.72 \\
           & Sym. &                  Min. Key &            394.38 & 84.84 & 27.28 & 24.64 &  14.53 &                     978.63 & 145.28 &        24.82 \\
\addlinespace
   \multirow{4}{*}{\shortstack{$\lpre \cdot 1.5$ if\\ speed \\ < 80kph}} &   Avg. &               Alternating &            361.83 & 19.50 & 10.92 & 10.94 &   5.34 &                     845.06 &  34.03 &        13.25 \\
           &   Avg. &                  Min. Key &            391.47 & 31.65 & 21.05 & 20.10 &  11.00 &                     917.13 &  52.23 &        23.78 \\
           & Sym. &               Alternating &            364.55 & 37.33 & 11.89 & 11.75 &   6.00 &                     836.44 &  57.93 &        11.53 \\
           & Sym. &                  Min. Key &            395.04 & 54.90 & 23.36 & 22.48 &  12.54 &                     908.12 &  84.33 &        22.01 \\
\bottomrule
\end{tabular}



==> table/cchpot_opts.tex <==
\begin{tabular}{ccccrrrrr}
\toprule
       & BCC & Deg2 & Deg3 & Zero & ALT & CH & CCH & Oracle \\
\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{\shortstack{Running\\time [ms]}}} & \xmark &        \xmark &        \xmark &  2\,133.0 &  317.9 &   47.9 &   54.4 &    34.3 \\
                                                                                    & \cmark &        \xmark &        \xmark &  1\,355.3 &  233.9 &   36.3 &   38.5 &    24.8 \\
                                                                                    & \cmark &         \cmark &        \xmark &   753.4 &  122.6 &   19.5 &   22.1 &    12.7 \\
                                                                                    & \cmark &         \cmark &         \cmark &   580.7 &   90.8 &   15.9 &   18.1 &    10.1 \\
\addlinespace
\multirow{4}{*}{\rotatebox[origin=c]{90}{\shortstack{Queue \\ {[$\cdot 10^3$]}}}} & \xmark &        \xmark &        \xmark &  8\,087.1 &  863.1 &  137.1 &  137.1 &   137.1 \\
                                                                                    & \cmark &        \xmark &        \xmark &  6\,298.2 &  685.7 &  112.7 &  112.7 &   112.7 \\
                                                                                    & \cmark &         \cmark &        \xmark &  2\,901.4 &  303.4 &   43.3 &   43.3 &    43.3 \\
                                                                                    & \cmark &         \cmark &         \cmark &  1\,681.4 &  179.7 &   26.8 &   26.8 &    26.8 \\
\bottomrule
\end{tabular}



==> table/customization_ger.tex <==
\begin{tabular}{lrrrr}
\toprule
& \multicolumn{4}{c}{Germany [s]} \\ \cmidrule(lr){2-5}
Threads & Basic & Perfect & Construct &  Total \\
\midrule
1           &   3.22 &     3.59 &       1.52 &   8.32 \\
2           &   1.76 &     1.81 &       0.76 &   4.33 \\
4           &   1.05 &     0.96 &       0.41 &   2.42 \\
8           &   0.75 &     0.54 &       0.27 &   1.56 \\
16          &   0.55 &     0.29 &       0.24 &   1.08 \\
\bottomrule
\end{tabular}



==> table/repr_knn_overview.tex <==
\begin{tabular}{l@{\hskip2pt}rrrrrrrrrr}
\toprule
& \multicolumn{5}{c}{$|P| = 2^{12}, |B| = 2^{20}$} & \multicolumn{5}{c}{$|P| = 2^{14}, |B| = |V|$} \\ \cmidrule(l{2pt}r{2pt}){2-6}\cmidrule(l{2pt}r{2pt}){7-11}
& \multicolumn{2}{c}{selection} & \multicolumn{3}{c}{query time [$\mu$s]} & \multicolumn{2}{c}{Selection} & \multicolumn{3}{c}{Query time [$\mu$s]} \\ \cmidrule(l{3pt}r{3pt}){2-3}\cmidrule(l{3pt}r{3pt}){4-6}\cmidrule(l{3pt}r{3pt}){7-8}\cmidrule(l{3pt}r{3pt}){9-11}
& Space & Time & \multicolumn{3}{c}{POIs to be reported} & Space & Time & \multicolumn{3}{c}{POIs to be reported} \\
&  [MB] & [ms] & {$k = 1$} & {$k = 4$} & {$k = 8$} &  [MB] & {[ms]} & {$k = 1$} & {$k = 4$} & {$k = 8$} \\
\midrule
Dijk.       &   2.2 &      0.1 & 712\,763.1 & 723\,458.3 & 730\,865.8 &   2.2 &       0.2 &     165.6 &     665.7 &  1\,346.0 \\
CRP         &    -- &       -- &         -- &         -- &         -- &   0.0 &       8.0 &        -- &     640.0 &        -- \\
{[orig]}    &  72.0 &     12.5 &   3\,150.7 &   4\,704.7 &   6\,230.4 &  72.0 &      13.8 &     363.6 &     594.2 &     852.7 \\
{[ours]}    &   0.0 &      0.1 &      278.6 &      311.7 &      338.4 &   0.0 &       0.6 &     359.0 &     445.0 &     532.5 \\
LR          &   0.0 &      0.0 &   3\,157.3 &   3\,157.6 &   3\,158.8 &   0.0 &       0.0 & 44\,441.2 & 44\,442.1 & 44\,451.0 \\
BCCH        &  89.7 &    324.6 &       25.8 &       27.8 &       29.5 & 141.5 &  1\,327.3 &       7.4 &      12.5 &      16.6 \\
\bottomrule
\end{tabular}



==> table/turn_opts.tex <==
\begin{tabular}{llrrrrrr}
\toprule
 &         &     CCH Edges & Prepro. & \multicolumn{2}{c}{Customization [ms]} & \multicolumn{2}{c}{Query [$\mu$s]} \\ \cmidrule(lr){5-6} \cmidrule(lr){7-8}
 &         & [$\cdot 10^3$] &   [s] & Basic & Perfect &  Basic & Perfect \\
\midrule
\multirow{7}{*}{\rotatebox[origin=c]{90}{Stuttgart}} & No turns &                    724.2 &             1.0 &                                        6.4 &                                          6.1 &   22.0 &   13.7 \\
       & CCH-Pot. &                    724.2 &             1.0 &                                        6.4 &                                          6.1 &    -- &  441.0 \\
       & Naive exp. &                   3\,214.9 &             3.6 &                                       18.0 &                                         23.4 &   55.7 &   25.3 \\
       & Cut order &                   3\,359.7 &             1.5 &                                       17.4 &                                         22.5 &   54.3 &   25.8 \\
       & Infinity &                   2\,874.6 &             1.6 &                                       16.5 &                                         20.1 &   53.4 &   26.0 \\
       & Directed &                   1\,550.5 &             1.6 &                                       13.2 &                                         16.2 &   40.0 &   26.4 \\
       & Reorder &                   1\,440.8 &             1.6 &                                       11.1 &                                         13.0 &   28.9 &   25.4 \\
\addlinespace \multirow{7}{*}{\rotatebox[origin=c]{90}{Germany}} & No turns &                  93\,443.1 &           220.3 &                                      552.1 &                                        541.4 &  426.9 &  155.4 \\
       & CCH-Pot. &                  93\,443.1 &           220.3 &                                      552.1 &                                        541.4 &    -- & 1\,659.5 \\
       & Naive exp. &                 440\,812.8 &          2\,087.7 &                                     2\,295.5 &                                       3\,131.0 & 1\,221.3 &  289.4 \\
       & Cut order &                 467\,191.1 &           371.1 &                                     2\,733.2 &                                       3\,400.6 & 1\,427.9 &  361.0 \\
       & Infinity &                 388\,201.7 &           390.3 &                                     2\,658.8 &                                       2\,858.1 & 1\,438.6 &  365.0 \\
       & Directed &                 206\,970.0 &           391.7 &                                     1\,760.9 &                                       2\,541.8 &  938.8 &  371.4 \\
       & Reorder &                 190\,597.1 &           391.4 &                                     1\,360.7 &                                       1\,899.2 &  647.6 &  378.0 \\
\addlinespace \multirow{7}{*}{\rotatebox[origin=c]{90}{Europe}} & No turns &                 117\,727.5 &           367.0 &                                      587.6 &                                        666.5 &  297.0 &  135.1 \\
       & CCH-Pot. &                 117\,727.5 &           367.0 &                                      587.6 &                                        666.5 &    -- & 2\,691.9 \\
       & Naive exp. &                 692\,995.8 &          3\,817.5 &                                     3\,169.9 &                                       4\,629.9 &  908.3 &  247.7 \\
       & Cut order &                 737\,433.4 &           407.5 &                                     3\,210.3 &                                       4\,670.8 &  928.8 &  264.8 \\
       & Infinity &                 651\,921.7 &           435.2 &                                     3\,257.5 &                                       4\,451.7 &  951.8 &  265.0 \\
       & Directed &                 363\,663.3 &           434.6 &                                     2\,184.1 &                                       3\,365.7 &  618.1 &  264.8 \\
       & Reorder &                 334\,755.9 &           436.7 &                                     1\,819.9 &                                       2\,663.0 &  453.1 &  295.8 \\
\bottomrule
\end{tabular}



==> table/turn_opts_ext.tex <==
\begin{tabular}{llrrrrrrrr}
\toprule
 &         &     CCH Edges & Prepro. & \multicolumn{4}{c}{Customization [ms]} & \multicolumn{2}{c}{Query [$\mu$s]} \\ \cmidrule(l{4pt}r{4pt}){5-8} \cmidrule(l{4pt}r{4pt}){9-10}
 &         & [$\cdot 10^3$] &           [s] & \multicolumn{2}{c}{Basic} & \multicolumn{2}{c}{Perfect} & Basic & Perfect \\ \cmidrule(l{4pt}r{4pt}){5-6} \cmidrule(l{4pt}r{4pt}){7-8}
 & Threads &                &               & 1 & 16 & 1 & 16 \\
\midrule
\multirow{7}{*}{\rotatebox[origin=c]{90}{Chicago}} & No turns &                    235.7 &             0.9 &                                             7.4 &                                              3.9 &                                              13.3 &                                                3.0 &   20.6 &   11.1 \\
       & CCH-Pot. &                    235.7 &             0.9 &                                             7.4 &                                              3.9 &                                              13.3 &                                                3.0 &    -- &  485.0 \\
       & Naive exp. &                   1\,637.2 &             1.3 &                                            64.7 &                                             21.9 &                                             133.2 &                                               15.5 &   72.0 &   27.1 \\
       & Cut order &                   1\,703.9 &             1.5 &                                            65.6 &                                             23.1 &                                             134.9 &                                               15.7 &   71.6 &   29.2 \\
       & Infinity &                   1\,571.9 &             1.5 &                                            70.3 &                                             19.2 &                                             104.9 &                                               14.6 &   70.9 &   29.3 \\
       & Directed &                    873.5 &             1.5 &                                            38.4 &                                             11.6 &                                             103.3 &                                               16.4 &   40.4 &   40.4 \\
       & Reorder &                    737.0 &             1.5 &                                            27.8 &                                              7.2 &                                              66.0 &                                                8.5 &   29.6 &   35.6 \\
% \multirow{7}{*}{\rotatebox[origin=c]{90}{London}} & No turns &                    363.7 &             0.6 &                                             9.9 &                                              3.5 &                                              16.6 &                                                3.0 &   20.9 &   11.8 \\
%        & CCH-Pot. &                    363.7 &             0.6 &                                             9.9 &                                              3.5 &                                              16.6 &                                                3.0 &    -- &  720.5 \\
%        & Naive exp. &                   1\,534.2 &             1.1 &                                            48.0 &                                             15.2 &                                             108.2 &                                               12.3 &   58.9 &   22.3 \\
%        & Cut order &                   1\,680.5 &             1.5 &                                            53.7 &                                             16.5 &                                             114.8 &                                               13.0 &   61.1 &   26.0 \\
%        & Infinity &                   1\,447.7 &             1.5 &                                            51.8 &                                             13.9 &                                              82.5 &                                               11.3 &   60.3 &   26.0 \\
%        & Directed &                    785.2 &             1.5 &                                            33.1 &                                              8.8 &                                              75.1 &                                               10.7 &   37.0 &   33.5 \\
%        & Reorder &                    697.6 &             1.5 &                                            26.3 &                                              6.2 &                                              53.0 &                                                7.0 &   26.1 &   31.4 \\
% \addlinespace \multirow{7}{*}{\rotatebox[origin=c]{90}{Stuttgart}} & No turns &                    724.2 &             0.9 &                                            15.9 &                                              3.9 &                                              24.5 &                                                3.8 &   17.5 &   10.2 \\
%        & CCH-Pot. &                    724.2 &             0.9 &                                            15.9 &                                              3.9 &                                              24.5 &                                                3.8 &    -- &  321.1 \\
%        & Naive exp. &                   3\,214.9 &             2.4 &                                            72.8 &                                             14.0 &                                             158.4 &                                               16.6 &   44.2 &   18.0 \\
%        & Cut order &                   3\,359.7 &             1.1 &                                            74.9 &                                             13.8 &                                             159.9 &                                               17.3 &   42.7 &   18.1 \\
%        & Infinity &                   2\,874.6 &             1.2 &                                            69.4 &                                             11.7 &                                             121.3 &                                               13.8 &   42.2 &   18.2 \\
%        & Directed &                   1\,550.5 &             1.2 &                                            52.8 &                                              9.1 &                                             104.0 &                                               12.0 &   26.8 &   22.3 \\
%        & Reorder &                   1\,440.8 &             1.2 &                                            47.2 &                                              7.5 &                                              82.8 &                                                9.2 &   19.3 &   21.3 \\
% \addlinespace \multirow{7}{*}{\rotatebox[origin=c]{90}{Germany}} & No turns &                  93\,443.1 &           165.6 &                                          2\,883.3 &                                            937.9 &                                            4\,696.1 &                                              628.3 &  330.8 &  104.6 \\
%        & CCH-Pot. &                  93\,443.1 &           165.6 &                                          2\,883.3 &                                            937.9 &                                            4\,696.1 &                                              628.3 &    -- & 1\,359.3 \\
%        & Naive exp. &                 440\,812.8 &          1\,584.6 &                                         14\,425.8 &                                           3\,238.3 &                                           31\,005.2 &                                             3\,194.1 &  953.9 &  192.0 \\
%        & Cut order &                 467\,191.1 &           299.0 &                                         15\,097.5 &                                           3\,747.9 &                                           32\,568.6 &                                             3\,521.3 & 1\,103.3 &  234.4 \\
%        & Infinity &                 388\,201.7 &           318.5 &                                         15\,174.2 &                                           3\,339.2 &                                           24\,890.1 &                                             2\,975.8 & 1\,104.3 &  234.5 \\
%        & Directed &                 206\,970.0 &           319.6 &                                          9\,754.1 &                                           2\,403.7 &                                           23\,459.0 &                                             2\,573.2 &  586.0 &  337.6 \\
%        & Reorder &                 190\,597.1 &           319.8 &                                          8\,273.4 &                                           2\,050.3 &                                           17\,331.0 &                                             2\,018.6 &  408.2 &  347.9 \\
% \addlinespace \multirow{7}{*}{\rotatebox[origin=c]{90}{Europe Turns}} & No turns &                 107\,042.6 &           202.3 &                                          3\,095.6 &                                           1\,092.0 &                                            5\,479.4 &                                              763.1 &  246.8 &  102.3 \\
%        & CCH-Pot. &                 107\,042.6 &           202.3 &                                          3\,095.6 &                                           1\,092.0 &                                            5\,479.4 &                                              763.1 &    -- & 3\,783.6 \\
%        & Naive exp. &                 622\,426.7 &          2\,474.0 &                                         17\,759.1 &                                           4\,041.4 &                                           38\,486.3 &                                             4\,070.2 &  712.3 &  170.4 \\
%        & Cut order &                 663\,587.3 &           300.3 &                                         18\,112.5 &                                           3\,983.6 &                                           38\,566.7 &                                             4\,126.7 &  786.8 &  190.9 \\
%        & Infinity &                 585\,062.3 &           319.3 &                                         18\,424.2 &                                           3\,590.4 &                                           32\,506.1 &                                             3\,686.3 &  781.7 &  190.5 \\
%        & Directed &                 326\,627.9 &           322.7 &                                         12\,693.0 &                                           2\,747.8 &                                           29\,559.5 &                                             3\,137.0 &  419.8 &  273.5 \\
%        & Reorder &                 302\,307.5 &           323.1 &                                         10\,620.0 &                                           2\,331.7 &                                           22\,436.9 &                                             2\,588.7 &  301.8 &  304.5 \\
% \addlinespace \multirow{7}{*}{\rotatebox[origin=c]{90}{Europe}} & No turns &                 117\,727.5 &           263.5 &                                          3\,366.5 &                                            982.4 &                                            6\,070.5 &                                              767.8 &  189.3 &   89.1 \\
%        & CCH-Pot. &                 117\,727.5 &           263.5 &                                          3\,366.5 &                                            982.4 &                                            6\,070.5 &                                              767.8 &    -- & 2\,311.1 \\
%        & Naive exp. &                 692\,995.8 &          2\,873.9 &                                         19\,670.2 &                                           3\,590.2 &                                           43\,816.2 &                                             4\,523.2 &  575.6 &  159.3 \\
%        & Cut order &                 737\,433.4 &           327.2 &                                         20\,082.1 &                                           3\,567.5 &                                           44\,365.9 &                                             4\,597.9 &  584.4 &  167.9 \\
%        & Infinity &                 651\,921.7 &           355.1 &                                         20\,145.2 &                                           3\,721.1 &                                           36\,436.2 &                                             3\,918.9 &  582.7 &  167.2 \\
%        & Directed &                 363\,663.3 &           359.7 &                                         13\,797.5 &                                           2\,808.6 &                                           33\,040.0 &                                             3\,495.1 &  645.8 &  260.9 \\
%        & Reorder &                 334\,755.9 &           357.0 &                                         11\,686.7 &                                           2\,450.2 &                                           25\,097.4 &                                             2\,889.0 &  469.0 &  299.2 \\
\bottomrule
\end{tabular}



==> table/turn_opts_ext2.tex <==
\begin{tabular}{ll@{\hskip3pt}rrrrrrrr}
\toprule
 &         &     CCH Edges & Prepro. & \multicolumn{4}{c}{Customization [ms]} & \multicolumn{2}{c}{Query [$\mu$s]} \\ \cmidrule(l{4pt}r{4pt}){5-8} \cmidrule(l{4pt}r{4pt}){9-10}
 &         & [$\cdot 10^3$] &           [s] & \multicolumn{2}{c}{Basic} & \multicolumn{2}{c}{Perfect} & Basic & Perfect \\ \cmidrule(l{4pt}r{4pt}){5-6} \cmidrule(l{4pt}r{4pt}){7-8}
 & Threads &                &               & 1 & 16 & 1 & 16 \\
\midrule
% \multirow{7}{*}{\rotatebox[origin=c]{90}{Chicago}} & No turns &                    235.7 &             0.9 &                                             7.4 &                                              3.9 &                                              13.3 &                                                3.0 &   20.6 &   11.1 \\
%        & CCH-Pot. &                    235.7 &             0.9 &                                             7.4 &                                              3.9 &                                              13.3 &                                                3.0 &    -- &  485.0 \\
%        & Naive exp. &                   1\,637.2 &             1.3 &                                            64.7 &                                             21.9 &                                             133.2 &                                               15.5 &   72.0 &   27.1 \\
%        & Cut order &                   1\,703.9 &             1.5 &                                            65.6 &                                             23.1 &                                             134.9 &                                               15.7 &   71.6 &   29.2 \\
%        & Infinity &                   1\,571.9 &             1.5 &                                            70.3 &                                             19.2 &                                             104.9 &                                               14.6 &   70.9 &   29.3 \\
%        & Directed &                    873.5 &             1.5 &                                            38.4 &                                             11.6 &                                             103.3 &                                               16.4 &   40.4 &   40.4 \\
%        & Reorder &                    737.0 &             1.5 &                                            27.8 &                                              7.2 &                                              66.0 &                                                8.5 &   29.6 &   35.6 \\
% \addlinespace
\multirow{7}{*}{\rotatebox[origin=c]{90}{London}} & No turns &                    363.7 &             0.6 &                                             9.9 &                                              3.5 &                                              16.6 &                                                3.0 &   20.9 &   11.8 \\
       & CCH-Pot. &                    363.7 &             0.6 &                                             9.9 &                                              3.5 &                                              16.6 &                                                3.0 &    -- &  720.5 \\
       & Naive exp. &                   1\,534.2 &             1.1 &                                            48.0 &                                             15.2 &                                             108.2 &                                               12.3 &   58.9 &   22.3 \\
       & Cut order &                   1\,680.5 &             1.5 &                                            53.7 &                                             16.5 &                                             114.8 &                                               13.0 &   61.1 &   26.0 \\
       & Infinity &                   1\,447.7 &             1.5 &                                            51.8 &                                             13.9 &                                              82.5 &                                               11.3 &   60.3 &   26.0 \\
       & Directed &                    785.2 &             1.5 &                                            33.1 &                                              8.8 &                                              75.1 &                                               10.7 &   37.0 &   33.5 \\
       & Reorder &                    697.6 &             1.5 &                                            26.3 &                                              6.2 &                                              53.0 &                                                7.0 &   26.1 &   31.4 \\[2pt]

\multirow{7}{*}{\rotatebox[origin=c]{90}{Stuttgart}} & No turns &                    724.2 &             0.9 &                                            15.9 &                                              3.9 &                                              24.5 &                                                3.8 &   17.5 &   10.2 \\
       & CCH-Pot. &                    724.2 &             0.9 &                                            15.9 &                                              3.9 &                                              24.5 &                                                3.8 &    -- &  321.1 \\
       & Naive exp. &                   3\,214.9 &             2.4 &                                            72.8 &                                             14.0 &                                             158.4 &                                               16.6 &   44.2 &   18.0 \\
       & Cut order &                   3\,359.7 &             1.1 &                                            74.9 &                                             13.8 &                                             159.9 &                                               17.3 &   42.7 &   18.1 \\
       & Infinity &                   2\,874.6 &             1.2 &                                            69.4 &                                             11.7 &                                             121.3 &                                               13.8 &   42.2 &   18.2 \\
       & Directed &                   1\,550.5 &             1.2 &                                            52.8 &                                              9.1 &                                             104.0 &                                               12.0 &   26.8 &   22.3 \\
       & Reorder &                   1\,440.8 &             1.2 &                                            47.2 &                                              7.5 &                                              82.8 &                                                9.2 &   19.3 &   21.3 \\[2pt]

\multirow{7}{*}{\rotatebox[origin=c]{90}{Germany}} & No turns &                  93\,443.1 &           165.6 &                                          2\,883.3 &                                            937.9 &                                            4\,696.1 &                                              628.3 &  330.8 &  104.6 \\
       & CCH-Pot. &                  93\,443.1 &           165.6 &                                          2\,883.3 &                                            937.9 &                                            4\,696.1 &                                              628.3 &    -- & 1\,359.3 \\
       & Naive exp. &                 440\,812.8 &          1\,584.6 &                                         14\,425.8 &                                           3\,238.3 &                                           31\,005.2 &                                             3\,194.1 &  953.9 &  192.0 \\
       & Cut order &                 467\,191.1 &           299.0 &                                         15\,097.5 &                                           3\,747.9 &                                           32\,568.6 &                                             3\,521.3 & 1\,103.3 &  234.4 \\
       & Infinity &                 388\,201.7 &           318.5 &                                         15\,174.2 &                                           3\,339.2 &                                           24\,890.1 &                                             2\,975.8 & 1\,104.3 &  234.5 \\
       & Directed &                 206\,970.0 &           319.6 &                                          9\,754.1 &                                           2\,403.7 &                                           23\,459.0 &                                             2\,573.2 &  586.0 &  337.6 \\
       & Reorder &                 190\,597.1 &           319.8 &                                          8\,273.4 &                                           2\,050.3 &                                           17\,331.0 &                                             2\,018.6 &  408.2 &  347.9 \\[2pt]
 \multirow{7}{*}{\rotatebox[origin=c]{90}{Europe Turns}} & No turns &                 107\,042.6 &           202.3 &                                          3\,095.6 &                                           1\,092.0 &                                            5\,479.4 &                                              763.1 &  246.8 &  102.3 \\
       & CCH-Pot. &                 107\,042.6 &           202.3 &                                          3\,095.6 &                                           1\,092.0 &                                            5\,479.4 &                                              763.1 &    -- & 3\,783.6 \\
       & Naive exp. &                 622\,426.7 &          2\,474.0 &                                         17\,759.1 &                                           4\,041.4 &                                           38\,486.3 &                                             4\,070.2 &  712.3 &  170.4 \\
       & Cut order &                 663\,587.3 &           300.3 &                                         18\,112.5 &                                           3\,983.6 &                                           38\,566.7 &                                             4\,126.7 &  786.8 &  190.9 \\
       & Infinity &                 585\,062.3 &           319.3 &                                         18\,424.2 &                                           3\,590.4 &                                           32\,506.1 &                                             3\,686.3 &  781.7 &  190.5 \\
       & Directed &                 326\,627.9 &           322.7 &                                         12\,693.0 &                                           2\,747.8 &                                           29\,559.5 &                                             3\,137.0 &  419.8 &  273.5 \\
       & Reorder &                 302\,307.5 &           323.1 &                                         10\,620.0 &                                           2\,331.7 &                                           22\,436.9 &                                             2\,588.7 &  301.8 &  304.5 \\[2pt]
 \multirow{7}{*}{\rotatebox[origin=c]{90}{Europe}} & No turns &                 117\,727.5 &           263.5 &                                          3\,366.5 &                                            982.4 &                                            6\,070.5 &                                              767.8 &  189.3 &   89.1 \\
       & CCH-Pot. &                 117\,727.5 &           263.5 &                                          3\,366.5 &                                            982.4 &                                            6\,070.5 &                                              767.8 &    -- & 2\,311.1 \\
       & Naive exp. &                 692\,995.8 &          2\,873.9 &                                         19\,670.2 &                                           3\,590.2 &                                           43\,816.2 &                                             4\,523.2 &  575.6 &  159.3 \\
       & Cut order &                 737\,433.4 &           327.2 &                                         20\,082.1 &                                           3\,567.5 &                                           44\,365.9 &                                             4\,597.9 &  584.4 &  167.9 \\
       & Infinity &                 651\,921.7 &           355.1 &                                         20\,145.2 &                                           3\,721.1 &                                           36\,436.2 &                                             3\,918.9 &  582.7 &  167.2 \\
       & Directed &                 363\,663.3 &           359.7 &                                         13\,797.5 &                                           2\,808.6 &                                           33\,040.0 &                                             3\,495.1 &  645.8 &  260.9 \\
       & Reorder &                 334\,755.9 &           357.0 &                                         11\,686.7 &                                           2\,450.2 &                                           25\,097.4 &                                             2\,889.0 &  469.0 &  299.2 \\
\bottomrule
\end{tabular}


